Coding Schemes for Securing Cyber-Physical Systems Against Stealthy Data Injection Attacks

This paper considers a method of coding the sensor outputs in order to detect stealthy false data injection attacks. An intelligent attacker can design a sequence of data injection to sensors and actuators that pass the state estimator and statistical fault detector, based on knowledge of the system parameters. To stay undetected, the injected data should increase the state estimation errors while keep the estimation residues small. We employ a coding matrix to change the original sensor outputs to increase the estimation residues under intelligent data injection attacks. This is a low cost method compared with encryption schemes over all sensor measurements in communication networks. We show the conditions of a feasible coding matrix under the assumption that the attacker does not have knowledge of the exact coding matrix. An algorithm is developed to compute a feasible coding matrix, and, we show that in general, multiple feasible coding matrices exist. To defend against attackers who estimates the coding matrix via sensor and actuator measurements, time-varying coding matrices are designed according to the detection requirements. A heuristic algorithm to decide the time length of updating a coding matrix is then proposed.

==> active_control.tex <==
\section{Active monitor injection to increase detection rate}
\labe{sec:active_control}
Now we consider design a sequence of active monitor injection to the control input and increase the false data alarm rate under attack. Assume the active monitor injection model is:
\begin{align}
\tilde{u}_k=u_k+\delta_k, \ k=1, 2,\cdots, T, \delta_k \in \Delta U
\label{u}
\end{align}
where $\Delta U$ is the set of feasible $\delta_k$ such that
\begin{align}
\begin{split}
&\tilde{x}_{k+1}=A\tilde{x}_k+B\tilde{u}_k +w_k,\\
&\tilde{y}_k=C\tilde{x}_k +v_k,\\
&\text{with corresponding definition of}\  \tilde{\hat{x}}_k, \tilde{z}_k, \tilde{e}_k,
\label{actives}
\end{split}
\end{align}
$\sum \limits_{k=1}^{T} \|\tilde{y}_k - y_k\| \leq \epsilon$ (For infinite horizon injection, $T\to\infty$, $\lim \limits_{k\to \infty} \|\tilde{y}_k - y_k\| \leq \epsilon$), i.e., the normal system state state should not change much because of the control input injection $\delta_k$. 
\FM{The definition of "feasible $\delta_k$" can be other constraints based on different design requirements}

When system is under attack and we apply the active monitor control input~\eqref{u}, the system model is:
\begin{align}
\begin{split}
&\tilde{x}'[k+1]=\mathbf{A}\tilde{x}'_{k}+\mathbf{B}\tilde{u}'_{k}+\mathbf{B}^{a}\tilde{u}^{a}_{k}+w_{k},\\
&\tilde{y}'_{k}=\mathbf{C}\tilde{x}'_{k}+\Gamma y^{a}_{k}+v_{k},\\
&\text{with corresponding definition of}\  \tilde{\hat{x}}'_k, \tilde{z}'_k, \tilde{e}'_k.
\end{split}
\label{activeas}
\end{align}

Then with active monitor injection, the difference of residues between normal and attacked systems is:
\begin{align}
\Delta \tilde{z}_k = \tilde{z}'_k - \tilde{z}_k.
\end{align}
The system needs to maximize $\Delta \tilde{z}_k$ for increasing detection rate, while the deception false data injection can cause a large state error: 
\begin{align}
\begin{split}
\max_{\delta_k} \min_{B^a, u_k^a, \Gamma, y^a_k} \quad& \sum\limits_{k=1}^{T}\|\Delta \tilde{z}_k\|_2\\
\text{subject to}\quad& ~\eqref{actives}, ~\eqref{activeas},\  \Delta \tilde{z}_k = \tilde{z}'_k - \tilde{z}_k\\
\quad& \delta_k \in \Delta U, \ k=1,2,\cdots, T,\\
\quad& \sum\limits_{k=1}^{T}\|\tilde{x}'_k - \tilde{x}_k\| \geq a
\end{split}
\label{detect}
\end{align}

In the worst case, all sensors and actuators are compromised, the problem reduces to:
\begin{align}
\begin{split}
\max_{\delta_k} \min_{u_k^a, y^a_k} \quad& \sum\limits_{k=1}^{T}\|\Delta \tilde{z}_k\|_2\\
\text{subject to}\quad& ~\eqref{actives}, ~\eqref{activeas},\  \Delta \tilde{z}_k = \tilde{z}'_k - \tilde{z}_k\\
\quad& \delta_k \in \Delta U, \ k=1,2,\cdots, T,\\
\quad& \sum\limits_{k=1}^{T}\|\tilde{x}'_k - \tilde{x}_k\| \geq a, \ B^a=\mathbf{I}, \Gamma=\mathbf{I},
\end{split}
\label{detect}
\end{align}


==> actuator.tex <==
\section{Both sensors and actuators are compromised}
A necessary condition for~\eqref{attackmodel} to cause unbounded system state $x[k]$:
\begin{theorem}[\cite{falsedata}]
The reachable region $\mathcal{R}$ is unbounded only if there exists a vector $v \in \mathbb{R}^{n}$ and a matrix $L^{a} \in \mathbb{R}^{q\times n}$, such that\\
1. v is an eigenvector of $A+B^{a}L^{a}$, the corresponding eigenvalue of which is $\lambda$;\\
2. $Cv$ belongs to the column space of $\Gamma$ or $\lambda=0$.
\label{nece}
\end{theorem}


A necessary and sufficient condition for stealth attack when both sensors and actuators are attacked is provided by~\cite{accstealth}:
\begin{theorem}%[\cite{accstealth}]
For the given model~\eqref{attackmodel}, there exist a non-zeros attack pair sequence $u^a_{k},y^a_{k}, k\in \{1,2, \cdots\}$ which can cause the unbounded error while maintaining a small residue condition~\ref{residue}, if and only if 
\begin{align}
span\{CQ_{ca}\} \subset span\{\Gamma\}
\label{saspan}
\end{align}
where $Q_{ca}$ is the controllability matrix of the pair $(A,B^a)$. 
\label{saiff}
\end{theorem}



==> redundant.tex <==
\section{Redundant Controller/Sensor}
\subsection{random select controller/sensor}
Assume we have m controllers $(C_{1}, ..., C_{M})$, each designed by some stable or optimal requirement,  not necessarily resilient for attack. The advantage of redundant controllers/sensors is :  random pick controller can decrease the probability that the active controller is included in the nonzero element of $B^{a}, \Gamma$ (or the disclosure/disruption resource of the system,~\cite{attackmodel}). 

\textbf{Can we apply "access key" for actuators and sensors that every step only some keys are feasible?}
  
Consider an extreme case, at time k, the system uniformly pick one active controller and the attacker also uniformly pick one controller to compromise, no false data injection to sensors ($\Gamma = 0$), then the probability that the active controller is safe is $P=1-\mathbf{C}_{m}^{1}\times \frac{1}{m^{2}} = 1-\frac{1}{m}$, and actually we have $B^{a}=0$. The necessary condition for the existence of unbounded reachable region is:\\
1. v is an eigenvector of $A$, the corresponding eigenvalue of which is $\lambda$;\\
2. $Cv=0$ or $\lambda=0$.

Note that this depends on the system model~\eqref{system}, if the system is observable, then with at least probability $P = 1-\frac{1}{m}$ (since the theorem is a necessary condition) there is no attack $\zeta^{a}$ satisfies : $\|z\|_{k} \leq 1$ and $\lim_{k \to \infty} \|x\|=\infty$, which means the attacker must take a risk to be detected if it wants to bring large bias to the system.  
\section{How to define the probability of }

==> sen_act.tex <==
\section{Both Sensors and Actuators are vulnerable}
\label{sec:sen_act}
\begin{definition}
A Givens rotation is a $n\times n$ rotation matrix, with $1$'s on the diagonal, $0$'s elsewhere, except the intersections of the $i$th and $j$th rows and columns corresponding to a rotation in the $(i,j)$ plane in $n$ dimensions. It takes the following form
\begin{align}
G(i,\ j,\ \theta)=\begin{bmatrix}1&\cdots&0&\cdots&0&\cdots&0\\ \vdots &\ddots &\vdots& &\vdots& &\vdots \\ 
0&\vdots & c &\cdots & -s & \cdots &0 \\ \vdots & &\vdots&\ddots&\vdots& &\vdots \\
0&\cdots&s&\cdots&c&\cdots&0 \\ \vdots& &\vdots& &\vdots&\ddots&\vdots \\ 0&\cdots&0&\cdots&0&\cdots&1
\end{bmatrix},
\end{align}
where $c=\cos \theta$, $s=\sin \theta $ appear
\end{definition}

The dynamics of change of estimation error, residuals between the normal and compromised system is
\begin{align}
\begin{split}
&\Delta e_{k+1} = (A-KCA) \Delta e_{k} - Ky^{a}_{k+1},\\
&\Delta z_{k+1}=CA\Delta e_k+ y^a_k,
\end{split}
\end{align}


\subsection{When Sensor Networks Have Structural Constraints}
